Towards physics-informed neural networks for landslide prediction

For decades, solutions to regional scale landslide prediction have mostly relied on data-driven models, by definition, disconnected from the physics of the failure mechanism. The success and spread of such tools came from the ability to exploit proxy variables rather than explicit geotechnical ones, as the latter are prohibitive to acquire over broad landscapes. Our work implements a Physics Informed Neural Network (PINN) approach, thereby adding to a standard data-driven architecture, an intermediate constraint to solve for the permanent deformation typical of Newmark slope stability methods. This translates into a neural network tasked with explicitly retrieving geotechnical parameters from common proxy variables and then minimize a loss function with respect to the available coseismic landside inventory. The results are very promising, because our model not only produces excellent predictive performance in the form of standard susceptibility output, but in the process, also generates maps of the expected geotechnical properties at a regional scale. Such architecture is therefore framed to tackle coseismic landslide prediction, something that, if confirmed in other studies, could open up towards PINN-based near-real-time predictions.

==> macros.tex <==
% LATeX packages ----
\usepackage[english]{babel}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{bm}
\usepackage{soul}

\RequirePackage[OT1]{fontenc}
\usepackage{amsthm,amsmath,natbib}
\usepackage{array}
\usepackage{float}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage[dvipsnames]{xcolor}
\usepackage{color}
\RequirePackage[colorlinks,citecolor=PineGreen,urlcolor=Emerald,linkcolor=RubineRed]{hyperref}
\usepackage{alltt}
\usepackage{fancyvrb}
\usepackage{gensymb}
\usepackage{algorithm2e}
\usepackage{pdfpages}
\usepackage{multirow}
\usepackage{lineno}
\usepackage{colortbl}
\usepackage{ulem}

% LaTeX macros ----

% Margins
\setlength{\oddsidemargin}{-0.125in} \setlength{\topmargin}{-0.5in}
\setlength{\textwidth}{6.5in} \setlength{\textheight}{9in}

\setlength{\textheight}{9in} \setlength{\textwidth}{6.5in}
\setlength{\topmargin}{-36pt} \setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt} \tolerance=500

% Definitions
\def\iid{{\ {\buildrel \rm{iid}\over \sim}\ }}
\def\ind{{\ {\buildrel \rm{ind}\over \sim}\ }}
\def\dotsim{{\ {\buildrel \cdot\over \sim}\ }}
\def\TO#1{{\textcolor{orange}{(TO:) #1}}}
\def\HT#1{{\textcolor{cyan}{HT: #1}}}
\def\RH#1{{\textcolor{red}{RH: #1}}}
%\def\COMM#1{{\textcolor{red}{FG: #1}}}
\def\FG#1{{\textcolor{magenta}{FG: #1}}}
\def\LL#1{{\textcolor{teal}{(LL: #1)}}}
\def\R#1{{\color{red}\bf #1}}%
\def\rr#1{{\color{red} #1}}%
\def\pr{\text{Pr}}%
\def\dt{\text{d}}
\def\E{\text{E}}
\def\Ex{\mathbb{E}}
\def\ss{\mathbf{s}}
\definecolor{Lightgray}{RGB}{235,235,235}
\renewcommand{\vec}[1]{\boldsymbol{#1}}

%latex shortcuts ----
%By Thomas Opitz - taken over from Anthony Davison's "macros.tex" file.

%simple shortcuts
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}

\def\rm#1{\mathrm{#1}}
\def\rmd{\mathrm{d}}

\def\vhalf{\vspace{\stretch{0.5}}}
\def\vone{\vspace{\stretch{1}}}
\def\vtwo{\vspace{\stretch{2}}}
\def\vthree{\vspace{\stretch{3}}}

\def\pr{\mathrm{pr}}

\def\calA{{\mathcal A}}
\def\calB{{\mathcal B}}
\def\calC{{\mathcal C}}
\def\calD{{\mathcal D}}
\def\calE{{\mathcal E}}
\def\calF{{\mathcal F}}
\def\calG{{\mathcal G}}
\def\calH{{\mathcal H}}
\def\calI{{\mathcal I}}


\def\auml{{\"a}}
\def\euml{{\"e}}
\def\uuml{{\"u}}


%redefine commands
\def\bar#1{\overline{#1}}

% \def\half{{\textstyle{1\over 2}}}
% \def\third{{\textstyle{1\over 3}}}
% \def\quarter{{\textstyle{1\over 4}}}
% \def\sixth{{\textstyle{1\over 6}}}
% \def\frac#1#2{{\textstyle{#1\over#2}}}
% \def\Beta{{\rm B}}

% \def\argmin{{\rm argmin}}  
% \def\diag{{\rm diag}}  
% \def\mod{{\rm mod}}  
% \def\tr{{\rm tr}}
% \def\sign{{\rm sign}}
% \def\ow{{\rm otherwise}}  
% \def\obs{{\rm obs}}  
% \def\endex{{\hfill{\color{red}$\bullet$}\medskip}}
% \def\Endex{{\hfill{$\bullet$}\medskip}}
% \def\redbf#1{{\color{red}\bf #1}}%
% \def\red#1{{\color{red} #1}}%
% \def\white#1{{\color{black} #1}}%

% \DeclareSymbolFont{AMSb}{U}{msb}{m}{n}
% \DeclareMathSymbol{\Natural}{\mathbin}{AMSb}{"4E}
% \DeclareMathSymbol{\Integer}{\mathbin}{AMSb}{"5A}
% \DeclareMathSymbol{\Real}{\mathbin}{AMSb}{"52}
% \DeclareMathSymbol{\Rational}{\mathbin}{AMSb}{"51}
% \DeclareMathSymbol{\Imaginary}{\mathbin}{AMSb}{"49}
% \DeclareMathSymbol{\Complex}{\mathbin}{AMSb}{"43} 
% \DeclareMathSymbol{\Disk}{\mathbin}{AMSb}{"44} 
% \def\bi{\begin{itemize}}
% \def\ei{\end{itemize}}
% \def\bd{\begin{description}}
% \def\ed{\end{description}}
% \def\ben{\begin{enumerate}}
% \def\een{\end{enumerate}}
% \def\bv{\begin{verbatim}}
% \def\ev{\end{verbatim}}

% \def\bth{{$b{\rm th}$ }}
% \def\cth{{$c{\rm th}$ }}
% \def\dth{{$d{\rm th}$ }}
% \def\fth{{$f{\rm th}$ }}
% \def\gth{{$g{\rm th}$ }}
% \def\hth{{$h{\rm th}$ }}
% \def\ith{{$i{\rm th}$ }}
% \def\jth{{$j{\rm th}$ }}
% \def\kth{{$k{\rm th}$ }}
% \def\lth{{$l{\rm th}$ }}
% \def\mth{{$m{\rm th}$ }}
% \def\nth{{$n{\rm th}$ }}
% \def\pth{{$p{\rm th}$ }}
% \def\rth{{$r{\rm th}$ }}
% \def\sth{{$s{\rm th}$ }}
% \def\tth{{$t{\rm th}$ }}
% \def\uth{{$u{\rm th}$ }}
% \def\vth{{$v{\rm th}$ }}
% \def\wth{{$w{\rm th}$ }}

% \def\calA{{\mathcal A}}
% \def\calL{{\mathcal L}}
% \def\calB{{\mathcal B}}
% \def\calC{{\mathcal C}}
% \def\calD{{\mathcal D}}
% \def\calE{{\mathcal E}}
% \def\F{{\mathcal F}}
% \def\G{{\mathcal G}}
% \def\H{{\mathcal H}}
% \def\calH{{\mathcal H}}
% \def\IG{{\mathcal IG}}
% \def\cI{{\mathcal I}}
% \def\cP{{\mathcal P}}
% \def\calJ{{\mathcal J}}
% \def\calK{{\mathcal K}}
% \def\calM{{\mathcal M}}
% \def\calN{{\mathcal N}}
% \def\N{{\calN}}
% \def\calP{{\mathcal{P}}}
% \def\calO{{\mathcal{O}}}
% \def\calS{{\mathcal{S}}}
% \def\calI{{\mathcal{I}}}
% \def\calR{{\mathcal R}}
% \def\calT{{\mathcal T}}
% \def\calU{{\mathcal U}}
% \def\calV{{\mathcal V}}
% \def\calW{{\mathcal W}}
% \def\calX{{\mathcal X}}
% \def\calY{{\mathcal Y}}
% \def\calZ{{\mathcal Z}}
% \def\W{{\mathcal W}}
% \def\U{{\Upsilon}}
% \def\f{\frac}
% \def\l{{\lambda}}
% \def\d{{\delta}}
% \def\bX{{\bar X}}
% \def\s{{\sigma}}
% \def\p{{\partial}}
% \def\p{{d}}
% \def\v{{\varepsilon}}
% \def\dis{{\displaystyle}}
% \def\a{{\alpha}}
% \def\b{{\beta}}
% \def\hash{{\#}}
% \def\bar#1{{\overline{#1}}}
% \def\hat#1{{\widehat{#1}}}
% \def\barY{{\overline{Y}}}
% \def\barX{{\overline{X}}}
% \def\barZ{{\overline{Z}}}
% \def\barx{{\overline{x}}}
% \def\bary{{\overline{y}}}
% \def\barz{{\overline{z}}}
% \def\T{{ \mathrm{\scriptscriptstyle T} }}
% \def\mT{{ -\mathrm{\scriptscriptstyle T} }}
% \newcommand{\indep}{\perp\!\!\!\perp}
% \newcommand{\nindep}{\perp\!\!\!\perp\!\!\!\!\!\!/\;\;}

% \newcommand{\med}{{\rm med}}
% \newcommand{\card}{{\rm card}}
% % \newcommand{\do}{{\rm do}}
% \newcommand{\Splus}{\textsc{S-Plus}\ }
% %\newcommand{\R}{\texttt{R} }

% % statistical notation

% \def\rmi{{\rm i}}
% \def\pr{{\rm Pr}}
% \def\Pr{\pr}
% \def\E{{\rm E}}
% \def\Ev{{\rm Ev}}
% \def\var{{\rm var}}
% \def\cov{{\rm cov}}  
% \def\corr{{\rm corr}}  
% \def\Estar{{\rm E^*\thinspace}}
% \def\varstar{{\rm var^*\thinspace}}
% \def\covstar{{\rm cov^*\thinspace}}  
% \def\median{{\rm median}}  
% \def\cum{{\rm cum}}
% \def\IMSE{{\rm IMSE}}  
% \def\AIC{{\rm AIC}}  
% \def\BIC{{\rm BIC}}  
% \def\NIC{{\rm NIC}}  
% \def\AICc{{\rm AIC_c}}  
% \def\CV{{\rm CV}}  
% \def\GCV{{\rm GCV}}  
% \def\IQR{{\rm IQR}}  
% \def\MAD{{\rm MAD}}  
% \def\Lik{{L}}
% \def\logL{{\ell}}
% \def\RLik{{RL}}
% \def\logLp{{\ell_{\rm p}}}

% \def\Dto{{\ {\buildrel D\over \longrightarrow}\ }}
% \def\Pto{{\ {\buildrel P\over \longrightarrow}\ }}
% \def\rto{{\ {\buildrel r\over \longrightarrow}\ }}
% \def\2to{{\ {\buildrel 2\over \longrightarrow}\ }}
% \def\Wto{{\ {\buildrel W\over \longrightarrow}\ }}
% \def\psto{{\ {\buildrel \rm{p.s.}\over \longrightarrow}\ }}
% \def\asto{{\ {\buildrel \rm{a.s.}\over \longrightarrow}\ }}
% \def\iid{{\ {\buildrel \rm{iid}\over \sim}\ }}
% \def\ind{{\ {\buildrel \rm{ind}\over \sim}\ }}
% \def\dotsim{{\ {\buildrel \cdot\over \sim}\ }}
% %\def\sim{{\ {\sim}\ }}
% %\def\to{{\longrightarrow}}
% \def\Deq{{\ {\buildrel D\over =}\ }}
% \def\Eoneton{{$E_1,\ldots,E_n$}}
% %\def\T1ton{{$T_1,\ldots,T_n$}}
% \def\I1ton{{$I_1,\ldots,I_n$}}
% %\def\U1ton{{$U_1,\ldots,U_n$}}
% \def\X1ton{{$X_1,\ldots,X_n$}}
% \def\Y1ton{{$Y_1,\ldots,Y_n$}}
% \def\Z1ton{{$Z_1,\ldots,Z_n$}}
% \def\R1ton{{$R_1,\ldots,R_n$}}
% \def\e1ton{{$e_1,\ldots,e_n$}}
% \def\t1ton{{$t_1,\ldots,t_n$}}
% \def\x1ton{{$x_1,\ldots,x_n$}}
% \def\y1ton{{$y_1,\ldots,y_n$}}
% \def\z1ton{{$z_1,\ldots,z_n$}}
% %\def\r1ton{{$r_1,\ldots,r_n$}}

% % Journal abbreviations

% \def\AAP{\emph{Advances in Applied Probability}}
% \def\AnnProbab{\emph{Annals of Probability}}
% \def\AISM{\emph{Annals of the Institute of Statistical Mathematics}}
% \def\AMS{\emph{Annals of Mathematical Statistics}}
% \def\ApplStatist{\emph{Applied Statistics}}
% \def\AS{\emph{Annals of Statistics}}
% \def\B{\emph{Bernoulli}}
% \def\Bka{\emph{Biometrika}}
% \def\CJS{\emph{Canadian Journal of Statistics}}
% \def\CSDA{\emph{Computational Statistics \& Data Analysis}}
% \def\Eca{\emph{Econometrica}}
% \def\ISI{\emph{International Statistical Review}}
% \def\ISR{\emph{International Statistical Review}}
% \def\JAMA{\emph{Journal of the American Medical Association}}
% \def\JAP{\emph{Journal of Applied Probability}}
% \def\JASA{\emph{Journal of the American Statistical Association}}
% \def\JBES{\emph{Journal of Business \& Economic Statistics}}
% \def\JCGS{\emph{Journal of Computational and Graphical Statistics}}
% \def\JSCS{\emph{Journal of Statistical Computation and Simulation}}
% \def\JRSSA{\emph{Journal of the Royal Statistical Society series A}}
% \def\JRSSB{\emph{Journal of the Royal Statistical Society series B}}
% \def\JRSSD{\emph{The Statistician}}
% \def\SJS{\emph{Scandinavian Journal of Statistics}}
% \def\SPA{\emph{Stochastic Processes and their Applications}}
% \def\SM{\emph{Survey Methodology}}
% \def\SS{\emph{Statistical Science}}
% \def\TAS{\emph{The American Statistician}}
% \def\Tech{\emph{Technometrics}}
% \def\ZW{\emph{Z. Wahrsch. v. geb.}}
% \def\JC{\emph{Journal of Classification}}
% \def\PNAS{\emph{Proceedings of the National Academy of Science}}

% % utility macros

% \def\np{{\newpage}}
% \def\gap{{\vskip 0.3in}}
% \def\etal{{\sl et al.}} 
% \def\pound{{\it \$}}
% \def\apriori{{\sl a priori }}
% \def\examfoot{{\vfill\hfill{\bf Turn over}\eject}}
% \def\newtransparency{{\newpage}}
% \def\Section{{Section~}}
% \def\Sections{{Sections~}}
% \def\Pvalue{{P-value}}
% \def\Pvalues{{P-values}}

% \def\report#1{{\newpage\centerline{\bf #1}\smallskip}}

% % odds and ends

% \def\redbf#1{{\color{red}\bf #1}}%
% \def\Defn{\redbf{Definition:\ }}%
% \def\Thm#1{\redbf{Theorem #1:\ }}%
% \def\Ex#1{\redbf{Example #1:\ }}%
% \def\Note{\redbf{Note:\ }}%
% \def\Exercise#1{\redbf{Exercise #1:\ }}%
% \def\Ill{\redbf{Illustration:\ }}%
% \def\endex{{\hfill\redbf{$\bullet$}\smallskip}}
% \def\calP{{\mathcal{P}}}
% \def\calS{{\mathcal{S}}}
% \def\calI{{\mathcal{I}}}
% \def\eme{{\`eme}}
% \def\ere{{\`ere}}
% %\def\picbox#1#2{{\centerline{\psfig{figure=#1,height=#2pc}}}}%
% \def\picbox#1#2#3{{\centerline{\psfig{figure=#1,height=#2pc,angle=#3}}}}%
% \def\tt#1{{\texttt{#1}}}
% \def\Der#1{\textbf{D#1}}


